Word2VisualVec: Image and Video to Sentence Matching by Visual Feature Prediction

This paper strives to find the sentence best describing the content of an image or video. Different from existing works, which rely on a joint subspace for image / video to sentence matching, we propose to do so in a visual space only. We contribute Word2VisualVec, a deep neural network architecture that learns to predict a deep visual encoding of textual input based on sentence vectorization and a multi-layer perceptron. We thoroughly analyze its architectural design, by varying the sentence vectorization strategy, network depth and the deep feature to predict for image to sentence matching. We also generalize Word2VisualVec for matching a video to a sentence, by extending the predictive abilities to 3-D ConvNet features as well as a visual-audio representation. Experiments on four challenging image and video benchmarks detail Word2VisualVec's properties, capabilities for image and video to sentence matching, and on all datasets its state-of-the-art results.

==> captioning-result.tex <==



\begin{figure*}[tb!]
\centering\includegraphics[width=2\columnwidth]{visual-to-text}
\caption{Some vision to language matching results by this work.
The last row are the sentences matched by \videovec~with audio, showing that adding audio sometimes help describe acoustics, e.g. \textit{sea wave} and \textit{speak}. 
See more results in the supplementary material.
}\label{fig:caption-results}
\end{figure*}




\begin{comment}
\begin{table*} [tb!]
\renewcommand{\arraystretch}{1.3}
\caption{Image-to-Text results produced by the proposed \ourmodelit. 
Sentences outside the ground truth of each test image are marked with \ding{56}.  \xr{Add video-to-sentence results. Visualize the results in a better designed way.}}
\label{tab:caption-results}
\centering
%\scalebox{1}{}
%\begin{threeparttable}
   \scalebox{0.85}{
    \begin{tabular}{@{}|c| l |@{}}
    \toprule
     \textbf{Test image}    & \textbf{Top-5 retrieved sentences} \\
     \midrule
   \multirow{5}{*}{\raisebox{-0.5\totalheight}{\includegraphics[height=0.13\textwidth]{771048251}}}    & \ding{52} Orange striped kitten biting blonde girl on the nose \\
                            & \ding{52} A orange kitten biting the nose of a child \\
                            & \ding{52} A blonde child is being bitten on the nose by a little orange kitten \\
                            & \ding{52} A cat bites a humans nose \\
                            & \ding{56} Two brown bears touching, face to face, with mouths open \\ [8pt]
     \midrule
    \multirow{5}{*}{\raisebox{-0.5\totalheight}{\includegraphics[height=0.13\textwidth]{3514019869}}} & \ding{52} A dog jumps over an obstacle \\   
                            & \ding{56} A dog is jumping across an obstacle \\
                            & \ding{52} A dog jumps over a hurdle in the grass \\
                            & \ding{56} A dog jumps over a read and blue hurdle \\
                            & \ding{56} A dog jumps over a hurdle at a competition \\   [8pt]
     \midrule
     \multirow{5}{*}{\raisebox{-0.5\totalheight}{\includegraphics[height=0.13\textwidth]{2251747182}}}  & \ding{56} A basketball game \\
                            & \ding{56} The Miami basketball player is looking \\
                            & \ding{56} The basketball player in white holds the ball \\
                            & \ding{56} The boy is playing basketball \\
                            & \ding{56} Miami basketball player shooting \\   [8pt] 
    \midrule                         
    \multirow{5}{*}{\raisebox{-0.5\totalheight}{\includegraphics[height=0.13\textwidth]{3255482333}}} & \ding{56} A skier about to go down the mountain \\
    &  \ding{52} A man is skiing down a mountain\\
    & \ding{56} A mountain skier heads down a mountain \\
    & \ding{56} a skier dressed in black speeds down the mountain \\
    & \ding{56} A skier catches air over the snow \\[8pt]

   \midrule                         
    \multirow{5}{*}{\raisebox{-0.5\totalheight}{\includegraphics[height=0.13\textwidth]{2460797929}}} & \ding{52} Boys in life jackets on a watercraft \\
    &  \ding{52} A group of people on a boat \\
    & \ding{52} A group of 6 boys are wearing yellow life vests and are on a make-shift raft \\
    & \ding{52} Several young people in life jackets are sitting on something floating in water \\
    & \ding{56} Several people are rowing a boat while being cheered on by a person with a drum \\[8pt]                                                          
 
    \bottomrule
    \end{tabular}
    }
%\end{threeparttable}
\end{table*}
\end{comment}


